Sparse Signal Detection in Heteroscedastic Gaussian Sequence Models: Sharp Minimax Rates

Given a heterogeneous Gaussian sequence model with unknown mean $\theta \in \mathbb R^d$ and known covariance matrix $\Sigma = \operatorname{diag}(\sigma_1^2,\dots, \sigma_d^2)$, we study the signal detection problem against sparse alternatives, for known sparsity $s$. Namely, we characterize how large $\epsilon^*>0$ should be, in order to distinguish with high probability the null hypothesis $\theta=0$ from the alternative composed of $s$-sparse vectors in $\mathbb R^d$, separated from $0$ in $L^t$ norm ($t \in [1,\infty]$) by at least $\epsilon^*$. We find minimax upper and lower bounds over the minimax separation radius $\epsilon^*$ and prove that they are always matching. We also derive the corresponding minimax tests achieving these bounds. Our results reveal new phase transitions regarding the behavior of $\epsilon^*$ with respect to the level of sparsity, to the $L^t$ metric, and to the heteroscedasticity profile of $\Sigma$. In the case of the Euclidean (i.e. $L^2$) separation, we bridge the remaining gaps in the literature.

==> contents/Conclusion.tex <==
\subsection{Conclusion and future work}
In this paper, we solved the problem of sparse signal detection in the heteroscedastic Gaussian sequence model with a diagonal matrix $\Sigma$, for any $L^t$ separation, $t\geq 1$. 
The natural and important case of a general covariance matrix $\Sigma$, not necessarily diagonal, stands out as a highly non-trivial extension of our results, but goes far beyond the scope of this paper. 
Another avenue of research for future work would be to translate the present results concerning the heteroscedastic Gaussian sequence model to the setting of testing sparse linear regression with non-isotropic design, generalizing~\cite{ingster2010detection}. 



==> contents/Ideas.tex <==

\begin{itemize}
    %\item Motivation: what is the point of sparse testing: inverse problems?
    %\item Not explicit expression
    %\item A fortiori if $\Sigma$  not diagonal: beyond scope
    %\item interpolation between $1$ and $2$: my papers
    %\item $L^2$ simpler but can be understood as particular case as the first two regimes coincide (dense parts).
    %\item In $L^1$: Valiant and Rajarshi in global
    %\item $\ell^1$ useful for testing discrete distributions as it is the total variation: future work.
    %\item other $L^t$ norms
    %\item In blockwise and link with Baraud
    %\item Link with Laurent, Loubes, Marteau but discuss differences 
    \item Sparse test: reminiscent of Sacha's ones + paper for estimating $L^\gamma$ norm. Difference: we don't need best polynomial approximation of too large order as we don't estimate the $L^t$ norm on $\R^d$ but just on the boundary of the testing pb.
    %\item Explain different regimes: discuss phase transition depending on the value of the sparsity parameter
    %\item In $L^2$ sparsity doesn't help when $s \gtrsim \sqrt{d}$, but in any other $L^t$ norm for $t<2$ it does.
    %\item Intermediate regime: show that in $\ell_1$ it it $\sqrt{s} \left(\displaystyle\sum_{i_*+1}^{j_*} \sigma_j^4\right)^{1/4}$
    \item upper bound: explain how we can guess the weights from the lower bound?
    %\item Truncation in the sparse test: $\tau$ and not just $2\lambda$ as in Sacha's paper.
    %\item $s\geq $ cst: artifact of the proof, should not be a requirement.
    %\item The paper~\cite{chhor2022sharp} studies the following problem.     We fix two discrete distributions $p,q$ over $\{1,\dots, d\}$, and consider an observation $X$ following a multinomial distribution $\mathcal{M}(n,q)$ for $n\in \N^*$.     We assume that $p$ is known and $q$ is unknown, and one aims at testing $q = p$ against $\|p-q\|_t \geq \epsilon$.     In this problem, the minimax separation radius $\epsilon^*(n,t,p)$ involves the $\ell_r$ norm of a sub-vector of $p$, where $r = \frac{2t}{4-t}$. The link with the present result is that the quantity $\sqrt{\frac{p_j}{n}}$ plays the role of $\sigma_j$, so that $\|p\|_r$ is proportional to $\left\|\frac{p}{n}\right\|_a$.     Note that when $t \to 2$, we have $a \to 4$, which recovers the dense contribution from Corollary~\ref{cor:rate_ell2}, except that $\lambda$ is defined in a slightly different way. 
    %Although Theorem~\ref{th:rate_ellt} encompasses the case where $t=2$, the method presented in Section~\ref{sec:results_ellt_>2} is more elegant in this special case.
    \item Not moment matching technique for too high order. In particular, don't have different phenomenon for even integers.
    %\item Rem: for $t>1$, csts dep on $t$, but not for $t \leq 2$ (compacity).
    %\item avenue for future work: regression.
\end{itemize}

==> contents/Results_ell2.tex <==
\section{Minimax rates in $L^2$ separation}\label{sec:results_ell2}
When $t=2$, the testing problem~\eqref{eq:testing_pb} can be rewritten as follows:
\begin{align}
    H_0: \theta = 0 \quad \text{ against } \quad H_1: \big\|\theta\big\|_2 \geq \epsilon \text{ and }
    \big\|\theta\big\|_0 \leq s.\label{eq:testing_pb_ell2}
\end{align}
The minimax separation radius $\epsilon^*(s,2,\Sigma)$ fundamentally depends on the value $\lambda_2$ defined below. 
Let $\beta \in \R$ be the unique solution to the equation
\begin{align}
    \frac{\sum_{j=1}^d \sigma_j^2 \exp\left(-\beta/\sigma_j^2\right)}{\sqrt{\sum_{j=1}^d \sigma_j^4 \exp\left(-\beta/\sigma_j^2\right)}} =
     \frac{s}{2}, \quad \text{ and let } \lambda_2 = \beta\lor 0.\label{eq:beta}
\end{align}
Note that equation~\eqref{eq:beta} always has a solution, since by Lemma~\ref{lem:monotonicity_t>2}, the left-hand side is continuous, strictly decreasing, tends to $+\infty$ as $\beta \to -\infty$ and tends to $0$ when $\beta \to +\infty$. 
The value $\lambda_2$ defined above does not admit an explicit expression for general profiles of $(\sigma_1,\dots, \sigma_d)$.
However, it is possible to explicitly find the value of $\beta$ up to constants for specific examples \ju{see examples}.
The expression of the minimax separation radius $\epsilon^*(s,2,\Sigma)$ is given as follows.
\begin{theorem}\label{th:rate_ell2}
Assume that $s \geq c(\eta)$ for some large enough constant $c(\eta)$ depending only on $\eta$. 
Let $\lambda_2$ be defined as in equation~\eqref{eq:beta}.
Then 
\begin{align}
    \epsilon^*(s,2,\Sigma)^2 \asymp  \lambda_2 s + \nu_2 \quad \text{ where } \nu_2 = \bigg(\sum_{j=1}^d\sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)\bigg)^{1/2}.\label{eq:implicit_separation_ell2}
\end{align}
This relation can be equivalently rewritten as follows. 
Let $j_* = \max\Big\{j \in [d]~\big|~ \sigma_j^2 \geq \lambda_2\Big\}$. Then we have
\begin{align}
    \epsilon^*(s,2,\Sigma)^2 \asymp \lambda_2 s + \Bigg(\sum_{j\leq j_*} \sigma_j^4\Bigg)^{1/2}. \label{eq:explicit_separation_ell2}
\end{align}
\end{theorem}
Theorem~\ref{th:rate_ell2} is proved by combining Propositions~\ref{prop:LB_gaussian_ell2} (lower bound) and~\ref{prop:UB_gaussian_ell2} (upper bound). 
The simplification in~\eqref{eq:explicit_separation_ell2} is proved in Lemma~\ref{lem:relations_between_contributions_ell>2} for general $t\geq 2$.
Equation~\eqref{eq:implicit_separation_ell2} will be useful to compare with Theorem~\ref{th:rate_ellt} and Theorem~\ref{th:rate_ellt_>2}, which respectively characterize the $L^t$ separation radius for $t\in [1,2]$ and $t \geq 1$. 
Equation~\eqref{eq:explicit_separation_ell2} is more convenient to interpret the result.
\begin{itemize}
    \item Theorem~\ref{th:rate_ell2} is best understood when compared with classical results on the isotropic case. 
    Assume that $\sigma_1 = \dots = \sigma_d =: \sigma$ and denote by $I_d$ the identity matrix of size $d$. 
    We know from~\cite{collier2017minimax} that in this case, 
    \begin{align*}
     \epsilon^*(s,2,\sigma^2 I_d) \asymp \begin{cases}\sigma d^{1/4} & \text{ if } s\geq \sqrt{d},\\
        \sigma \sqrt{s\log\left(1+d/s^2\right)}& \text{ otherwise.}\end{cases}
    \end{align*}
    In this expression, the elbow at $s \gtrless \sqrt{d}$ can be replaced by $s \gtrless c\sqrt{d}$ for any absolute constant~$c$ without affecting the rate, up to multiplicative constants depending only on $c$. 
    This result can be recovered from Theorem~\ref{th:rate_ell2} in the present paper. 
    Indeed, in the homoscedastic model, $\beta$ solves $\sqrt{d}\exp\left(-\beta/2\sigma^2\right) = s/2$, i.e. $\beta = \sigma^2 \log\left(\frac{2\sqrt{d}}{s}\right)$. 
    There are two cases.
    \begin{itemize}
        \item If $s> 2\sqrt{d}/e$, then $\sigma^2> \lambda_2$ and $j_* = d$.
    Therefore, equation~\eqref{eq:explicit_separation_ell2} yields that $\epsilon^*(s,2,\sigma^2 I_d) = \sigma d^{1/4}$. 
    \item Otherwise, if $s < 2\sqrt{d}/e$, then $\sigma^2\leq \lambda_2$ and $j=0$ so that the minimax separation radius scales as $\epsilon^*(s,2,\sigma^2 I_d) \asymp \sqrt{\lambda_2 s} \asymp \sigma \sqrt{s \log(1+d/s^2)}$. 
    \end{itemize}
    \item Noticeably, the isotropic case involves a brutal phase transition: we either have $j_*=0$  or $j_* = d$.
    In this case, all of the coordinates exclusively belong to the \textit{dense set of coordinates} $\{j \leq j_*\}$ or to the \textit{sparse set of coordinates} $\{j>j_*\}$.
    In the heteroscedastic model however, the phase transition is more subtle. 
    When $s =  d$, all of the coordinates contribute to the dense regime $\left(\sum_{j=1}^d \sigma_j^4\right)^{1/4}$. 
    However, when we let $s$ decrease from $d$ to $O_\eta(1)$, the cut-off $j_*$ progressively shifts from $d$ to $0$. 
    \item This smoother interpolation between the fully dense and fully sparse regimes is reflected in the fact that the minimax separation radius in $L^2$ generally involves two contributions. 
    We recall that in the fully dense case when $s=d$, the minimax separation radius $\epsilon(d,2)^2 $ is known to be $\left(\sum_{j=1}^d \sigma_j^4\right)^{1/2}$, see Propositions $1$ and $2$ in~\cite{laurent2012non}. 
    The part $\left(\sum_{j\leq j_*} \sigma_j^4\right)^{1/4}$ therefore represents the dense contribution, which we would obtain by only testing the first $j_*$ coordinates with a sparsity $s' = j_*$. 
    The second contribution in this rate corresponds to the term $\lambda_2 s$. 
    The term $\lambda_2$ is obtained by solving the equation~\eqref{eq:beta}, which does not admit explicit solutions as a function of the $\sigma_j$'s in the general case. 
    However, it is possible to solve equation~\eqref{eq:beta} for some specific profiles of $\Sigma$. \ju{see Examples}
    In the isotropic case, the term $\lambda_2 s$ is responsible for the rate $\sigma \sqrt{s\log(d/s^2)}$ when $s\gg \sqrt{d}$.
    \item When $\lambda_2 = 0$, which by Lemma~\ref{lem:monotonicity_t>2}, exactly corresponds to the condition $s/2 \geq  \frac{\sum_{j=1}^d \sigma_j^2}{\sqrt{\sum_{j=1}^d \sigma_j^4}}$, it holds that $\epsilon^*(s,2,\Sigma) = \epsilon^*(d,2,\Sigma)$. 
    In other words, sparsity does not help. 
    In the homoscedastic case, this phenomenon arises when $s\geq \sqrt{d}$. In the heteroscedastic case, the threshold $\sqrt{d}$ is replaced by the stable rank of $\Sigma$ defined as $\operatorname{Tr}(\Sigma) / \operatorname{Tr}^{1/2}(\Sigma^2)$.
    \end{itemize}
    
\subsection{Lower bound}
\begin{proposition}
\label{prop:LB_gaussian_ell2}
Assume that $s \geq c(\eta)$ and let $\lambda_2$ be defined as in equation~\eqref{eq:beta}.
Then there exists a small constant $c$ depending only on $\eta$, such that 
$$\epsilon^*(s,t,\Sigma) \geq  c\lambda_2 s{2} + c \sqrt{\sum_{j=1}^d\sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)}.$$
\end{proposition}
The proof is contained in the proof of Proposition~\ref{prop:LB_gaussian_ellt_>2}, which states the lower bound for general $t \geq 2$.
\vspace{1mm}

Our lower bound construction uses Le Cam's two points method, by defining a prior distribution over the parameter space $\Theta = \R^d$. 
We define a random vector $\theta \in \R^d$ whose coordinates $\theta_j$ satisfy $\forall j \in [d]: \theta_j = b_j \omega_j \gamma_j$, where $b_j \sim \operatorname{Ber}(\pi_j)$, $\omega_j \sim \operatorname{Rad}(\frac{1}{2})$ are mutually independent, and
\begin{align}
    \pi_j &= \frac{\sigma_j^2 \exp\left(-\lambda_2/\sigma_j^2\right)}{\sqrt{\sum_{j=1}^d \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)}},\label{eq:pi_j}\\
    \gamma_j &= \sigma_j \arg \sinh^\frac{1}{2} \left[c \cdot \exp\left(\lambda_2/\sigma_j^2\right)\right] \asymp \sigma_j + \sqrt{\lambda_2},\label{eq:gamma_j}
\end{align} 
for some small enough $c$ depending only on $\eta$. 
The magnitude $\gamma_j$ of the perturbation satisfies $\gamma_j \asymp \sigma_j$ if $j \leq j_*$, and $\gamma_j^2 \asymp \lambda_2$ if $j>j_*$. 
The perturbation $\gamma_j \asymp \sigma_j$ coincides with the optimal perturbation that one would set in absence of sparsity (see~\cite{laurent2012non}, proof of Proposition $1$).
The perturbation $\gamma_j \asymp \sqrt{\lambda_2}$ is more surprising, as it does not depend on $\sigma_j$.
This can be understood by noting that $\pi_j \propto \sigma_j^2 \exp\!\left(-\lambda_2/\sigma_j^2\right)$, which implies $\pi_1\geq \dots \geq \pi_d$, with a very fast decay of $\pi_j$ with $\sigma_j$ when $\sigma_j \ll \sqrt{\lambda_2}$. 
In other words, our sparse prior preferably selects coordinates with larger $\sigma_j$ to set the perturbation $\pm \gamma_j$. 
This makes intuitive sense: if $\sigma_j = 0$, then under $H_0$, we should observe $X_j = 0$ \textit{a.s.} so that it is optimal to choose $\pi_j=0$. 
This stands in contrast with the lower bound proposed in the paper~\cite{laurent2012non}, which also considers Problem~\eqref{eq:testing_pb_ell2}. 
In the latter paper, the prior is defined by perturbing some coordinates $\big\{\theta_j ~\big|~ j\in J \big\}$, for a set $J$ selected \textit{uniformly at random} among subsets of $[d]$ of cardinality $s$, leading to sub-optimality in specific regimes. 

\vspace{2mm}

Our lower bound requires the condition $s\geq c(\eta)$, which is not needed in the upper bound.
We conjecture that this is an artifact of the proof, and that the lower bound should hold for any $s\geq 1$. 
Indeed, our prior has a \textit{random} sparsity, equal to $\sum_{j=1}^d b_j$. 
Its expectation, $\sum_{j=1}^d \pi_j \leq s/2$ and its standard deviation $\sqrt{\sum_{j=1}^d  \pi_j(1-\pi_j)} \leq \sqrt{s}$, ensure by Chebyshev's inequality that our prior's sparsity is at most $s$ with probability $1-\eta/10$, provided that $s$ is greater than a constant depending only on $\eta$ (see equation~\eqref{eq:control_prior_sparsity}).
This non-deterministic sparsity requires using $s/2$ rather than $s$ in equation~\eqref{eq:beta}, which we believe could be replaced with $s$.
In the homoscedastic case~\cite{baraud2002non,laurent2012non,collier2017minimax, kotekal2021minimax}, the condition $s \geq c(\eta)$ is never needed in the lower bound, as the sparse support of $\theta$ is drawn uniformly at random among all families of $s$ elements in $\{1,\dots,d\}$. 
In our case, imposing a prior sparsity exactly equal to $s$ would require drawing $s$ coordinates in $\{1,\dots,d\}$ \textit{without replacement}, each coordinate $j$ being selected with probability proportional to $\pi_j$. 
    
    
\subsection{Upper bound}

We now describe the tests achieving the rate in Theorem~\ref{th:rate_ell2}. 
Let $\lambda_2$ be defined as in equation~\eqref{eq:beta} and let 
\begin{align}
    \uptau_2 = 2 \lambda_2 + \nu_2/s \quad \text{ where } \quad \nu_2 = \Bigg(\sum_{j=1}^d \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)\Bigg)^{1/2}. \label{eq:def_nu}
\end{align}
For any $j >j_*$, let also 
\begin{align}
    \alpha_j := \mathbb E \left[Z_j^2 \,\big|\, Z_j^2  >  \uptau_2 \right] ~\text{where $Z_j \sim \mathcal{N}(0,\sigma_j^2)$},
\end{align}
and now define the test statistics as follows:
\begin{align}
     T_{dense} = \sum_{j \leq j_*} X_j^2- \sigma_j^2, \quad \text{ and } \quad
    &T_{sparse} = \sum_{j > j_*} \big(X_j^2 - \alpha_j\big)\mathbb 1\left\{X_j^2 > \uptau_2\right\}. \label{eq:def_test_stat}
\end{align}
For some large enough constant $C$ depending only on $\eta$, we finally define the test function
\begin{align}
    \psi_{sparse} &= \mathbb 1\Big\{T_{sparse} > C\rho \Big\},\quad \psi_{dense} = \mathbb 1\Bigg\{T_{dense} \geq C \sqrt{\sum_{j \leq j_*} \sigma_j^4}\Bigg\},
    ~~ 
    \text{ and } 
    ~~
    \psi = \psi_{sparse} \lor \psi_{dense}\label{eq:def_tests}
    \\
    \text{ where } \rho & = \lambda_2 s +  \nu_2.\label{eq:def_rho}
\end{align}
We state the following Proposition which complements the lower bound from Proposition~\ref{prop:LB_gaussian_ell2} by a matching upper bound.
\begin{proposition}\label{prop:UB_gaussian_ell2}
Recall the definition of $\rho$ in~\eqref{eq:def_rho}. There exists a large enough constant $C'$ depending only on $\eta$ such that
\begin{align*}
\begin{cases}
    \mathbb P_\theta\left(\psi = 1\right) \leq \eta/2 & \text{ if } ~~ \theta=0,\\
    \mathbb P_\theta\left(\psi = 0\right)\leq \eta/2 & \text{ if } ~ \|\theta\|^2 \geq C' \rho.
\end{cases}  
\end{align*}
Therefore, $\epsilon^*(s,2,\Sigma)^2 \leq C'\left( \lambda_2 s + \nu_2\right)$.
\end{proposition}
The proof is omitted as it is encompassed in the proof of Proposition~\ref{prop:UB_gaussian_ellt_>2}, which gives the upper bound for any $t\geq 2$. 
We can compare this upper bound with the literature in the isotropic case~\cite{collier2017minimax}. 
When $\sigma_1 = \dots = \sigma_d =: \sigma$ the test statistic used in~\cite{collier2017minimax} is defined as follows
\begin{numcases}{T=}
    $$\sum\limits_{j=1}^d X_j^2 - \sigma^2 $$ & $ \text{ if } s > \sqrt{d}$,\label{eq:dense_test_isotropic}
    \\
    $$\sum\limits_{j=1}^d (X_j^2 - \alpha_s \sigma^2)\mathbb 1_{|X_j| > \sigma\sqrt{2\log(1+d/s^2)}}$$ &  $\text{ otherwise},$\label{eq:sparse_test_isotropic}
\end{numcases}
where $\alpha_s = \mathbb E\left[X^2 \,\big|\, X^2> 2\log(1+\frac{d}{s^2})\right]$.
We can compare this with our results.
As noticed above, when $s > \frac{2}{e}\sqrt{d}$, our result implies that $j_*=d$ and our dense test statistic coincides with~\eqref{eq:dense_test_isotropic}. 
When $s \leq \frac{2}{e} \sqrt{d}$, we have $j_* = 0$ and our sparse test coincides with~\eqref{eq:sparse_test_isotropic}. 
Contrary to~\cite{collier2017minimax}, our phase transition occurs at $s = \frac{2}{e} \sqrt{d}$ rather than $s=\sqrt{d}$, which only affects the multiplicative constants in the rates.
Note that from equations~\eqref{eq:dense_test_isotropic} and~\eqref{eq:sparse_test_isotropic}, the isotropic case requires only \textit{one} test at a time. 
This reflects the fact that the isotropic case never involves a superposition of two contributions in the rate, as~$j_*$ is always equal to~$0$ or to~$d$. 
In the present heteroscedastic case, however, the rate is a combination of two contribution with fundamentally different behaviors, which requires handling the two regimes simultaneously with two different tests.
\vspace{2mm}

Note that if $s \lesssim \sqrt{d}$, the isotropic sparse test~\eqref{eq:sparse_test_isotropic} requires the truncation $X_j^2 >2 \sigma^2 \log\!\big(1\!+\!\frac{d}{s^2}\big) \asymp 2 \lambda_2$. 
In comparison, our sparse test $T_{sparse}$ requires the truncation $X_j^2>\uptau_2$ where $\uptau_2 = 2\lambda_2 + \nu_2/s$, which is larger than~$2\lambda_2$. 
The reason is that setting $\uptau_2 = 2\lambda_2$ would cause  $\operatorname{Var}_{H_0}\!\left[T_{sparse}\right]$ to be too large when the dense regime dominates, that is, when $\nu_2 \gg \lambda_2 s$. 
However, when the sparse regime dominates, i.e. when $\nu_2 \lesssim \lambda_2 s$, we recover $\uptau_2 \asymp 2\lambda_2$. 
In the isotropic case~\cite{collier2017minimax}, truncating at $2\lambda_2$ is sufficient, since $\nu_2/s$ never dominates over $2\lambda_2$ when $s \lesssim \sqrt{d}$ (see Remark~\eqref{rem:isotropic}).

\ju{\begin{itemize}
    \item Compare with beatrice
\end{itemize}}




==> contents/Trash.tex <==
% Discussion: block-wise constant L2

\item Consider the case of block-wise constant variances: Assume that the family $(\sigma_1, \dots \sigma_d)$ can be split into $K$ blocks of indices $I_1, \dots, I_K$ such that for $K$ real numbers $\sigma_{\!I_1}, \dots, \sigma_{I_K} \geq  0$, we have $\forall k \in [K],\forall j \! \in \! I_k: \sigma_j = \sigma_{I_k}$.
    Assume furthermore that $K$ is a constant. 
    Then, by the Cauchy-Schwarz inequality, $\beta$ solves the equation 
    \begin{align*}
        \frac{s}{2} = \frac{\sum_{k=1}^K |I_k|\sigma_{I_k}^2 \exp\left(-\beta/\sigma_k^2\right)}{\sqrt{\sum_{k=1}^K |I_k|\sigma_{I_k}^4 \exp\left(-\beta/\sigma_k^2\right)}} \asymp_K \sqrt{\sum_{k=1}^K |I_k|\exp\left(-\beta/\sigma_k^2\right)} \asymp_K \sqrt{\max_{k=1}^K |I_k|\exp\left(-\beta/\sigma_k^2\right)},
    \end{align*}
    so that $\beta = \max\limits_{k \in [K]} \left\{ \sigma_k^2 \log\left(C_K\dfrac{|I_k|}{s^2}\right)\right\} $ for some constant $C_K$ depending only on $K$. 
    we can solve for lambda. As long as the number of blocks remains constant, Cauchy-Schwarz stays tight. However, when the number of blocks grows, this inequality fails to hold and we have to use the expression with the implicitly defined $\lambda$.
    
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Proof of equivalence: We have 
$$ \nu^t + \lambda^t s 
\asymp 
\left[\sum_{j \leq i_*} \sigma_j^{a}\right]^{t/a} 
+ \frac{1}{\lambda^{2-t}} \left(\sum_{j = i_*+1}^{j_*} \sigma_j^4\right)^{1/2} 
+ \lambda^t s \quad (why?)$$

and $$ \lambda^t s+\dfrac{1}{\lambda^{2-t}} \displaystyle\left[\sum\limits_{j>i_*}^{j_*} \sigma_j^4\right]^{1/2}  
\geq \inf_{\lambda' >0} (\lambda')^t s
+ \dfrac{1}{(\lambda')^{2-t}} \displaystyle\left[\sum\limits_{j>i_*}^{j_*} \sigma_j^4\right]^{1/2} 
= 2 s^{1-t/2} \left[\sum\limits_{j>i_*}^{j_*} \sigma_j^4\right]^{t/4},$$ 

so that 
\begin{align}
    \epsilon^*(s,t,\Sigma)^t \gtrsim \left\|\sigma_{\leq i_*}\right\|_a^t + \big\|\sigma_{int}\big\|_4^t\; s^{1-t/2} + \lambda^t s.\label{eq:variational_lambda}
\end{align}

To prove the converse inequality, we distinguish between two cases.
\begin{itemize}
    \item First case, if $\lambda^t s \geq \frac{1}{\lambda^{2-t}} \left(\sum\limits_{j = i_*+1}^{j_*} \sigma_j^4\right)^{1/2} $, then we have $\big\|\sigma_{int}\big\|_4^t\; s^{1-t/2} \leq \lambda^t s$
     \begin{align*}
        \epsilon^*(s,t,\Sigma)
        \asymp 
        \left[\sum_{j \leq i_*} \sigma_j^{a}\right]^{t/a} 
        + \frac{1}{\lambda^{2-t}} \left(\sum_{j = i_*+1}^{j_*} \sigma_j^4\right)^{1/2} 
        + \lambda^t s\\
     \end{align*}
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Surprisingly, the contribution of the intermediate regime $\big\|\sigma_{int}\big\|_4^t\; s^{1-t/2}$ never dominates. More precisely, in the proof of Theorem~\ref{th:rate_ellt}, we argue that if it dominates, then it must be of the same order as $\lambda^t s$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:relations_between_contributions_ell2}
We recall that $j_* = \max\big\{j\in[d] ~\big|~ \sigma_j^2 \geq \lambda_2\big\}$. We let
\begin{align*}
    \left\{\begin{array}{ll}
         s_{sparse} = \dfrac{1}{\nu_2}\sum_{j>j_*} \sigma_j^2 \exp\left(-\lambda_2/\sigma_j^2\right),\\[10pt]
         \nu_{sparse} = \sqrt{\sum_{j>j_*} \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)},\\[10pt]
         \nu_{dense} = \sqrt{\sum_{j>j_*} \sigma_j^4}.
    \end{array}\right.
\end{align*}
We have $\nu \asymp \nu_{dense} + \nu_{sparse}$. Moreover, we also have $\nu_{sparse}^2 \leq \nu_2 \lambda s_{sparse}$. In particular, it holds that $\nu_2 + \lambda_2 s = \nu_{dense} + \lambda_2 s$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:relations_between_contributions_ell2}]
By definition of $j_*$, the following relations are true up to absolute constants:
\begin{align*}
    \nu = \sqrt{\sum_{j=1}^d \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)} 
    &\asymp \sqrt{\sum_{j\leq j_*} \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)} + \sqrt{\sum_{j>j_*} \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)}\\ 
    &\asymp \sqrt{\sum_{j>j_*} \sigma_j^4 } + \sqrt{\sum_{j>j_*} \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right)}\\
    & = \nu_{dense} + \nu_{sparse}.
\end{align*}
Moreover, we have
\begin{align}
    \nu_{sparse}^2 = \sum_{j>j_*} \sigma_j^4 \exp\left(-\lambda_2/\sigma_j^2\right) \leq 
    \lambda_2 \sum_{j>j_*} \sigma_j^2 \exp\left(-\lambda_2/\sigma_j^2\right) = \nu_2 \lambda_2 s_{sparse}.\label{eq:relation_sparse_ell2}
\end{align}
We now prove that $\nu_2 + \lambda_2 s \asymp \nu_{dense} + \lambda_2 s$. 
If $\nu_{sparse} \leq \nu_{dense}$, this relation is clear. 
Otherwise, $\nu_2 \leq 2 \nu_{sparse}$ so that by~\eqref{eq:relation_sparse_ell2}, we have $\nu_{sparse}\leq 2 \lambda_2 s_{sparse}$. 
Therefore, $\nu_2\leq 2 \nu_{sparse} \leq 4 \lambda_2 s_{sparse} \leq 4 \lambda_2 s$, so that $\nu_2 + \lambda_2 s \asymp \lambda_2 s \asymp \nu_{dense} + \lambda_2 s$. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

we can use the same Taylor expansion as in~\eqref{eq:taylor}:
\begin{align*}
    \big|\theta_j + \xi_j\big|^\alpha 
    &= 
    |\theta_j|^\alpha 
    + \alpha \big|\theta_j^{\alpha-1} \xi_j\big| \operatorname{sign}(\theta_j \xi_j) 
    + \frac{\alpha (\alpha-1)}{2} \xi_j^2 \big|\theta_j + \xi'_j\big|^{\alpha-2}
    \\
    &
    \geq 
    |\theta_j|^\alpha 
    - \alpha \big|\theta_j^{\alpha-1} \xi_j\big|,
\end{align*}
for any $\alpha \geq 2$. Moreover,
\begin{align*}
    \mathbb E \left[|\theta_j|^t
    - t \big|\theta_j^{t-1} \xi_j\big|\right] = |\theta_j|^t
    - C \big|\theta_j^{t-1}\big| \sigma_j
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Justification $\sum \pi_j \leq s$
If $\beta<0$, then by definition of $\beta$, no $\beta'>\beta$ solves the equation~\eqref{eq:beta}, hence by continuity: 
\begin{align*}
    \forall\beta'>\beta:~~  \frac{\sum_{j=1}^d \sigma_j^t \exp\left(-\beta'/\sigma_j^2\right)}{\sqrt{\sum_{j=1}^d \sigma_j^{2t} \exp\left(-\beta'/\sigma_j^2\right)}} < \frac{s}{2}.
\end{align*}
In particular, this holds for $\beta'=0$, which ensures that $\sum_{j} \pi_j < s/2$.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

the interpretation of $j_*$ from the perspective of the lower bound. 
Indeed, as argued in the proof, the condition ensuring indistinguishability  of the prior is
\begin{align}
    \sum_{j=1}^d \pi_j^2 \sinh^2\left(\frac{\gamma_j^2}{2\sigma_j^2}\right) \leq c',
\end{align}
for a sufficiently small constant $c' = c'(\eta)$ (see equation~\eqref{eq:chi2}).
As evoked in Subsection~\ref{subsec:LB_t>2},  index $j_*$ is the largest index $j$ for which $\gamma_j \leq c \sigma_j$, allowing for the following simplifications: $\sinh\left(\gamma_j^2/2\sigma_j^2\right) \asymp \gamma_j^2/\sigma_j^2$ for $j \leq j_*$, and $\sinh^2\left(\gamma_j^2/2\sigma_j^2\right) \asymp \exp(\gamma_j^2/\sigma_j^2)$ for $j>j_*$. 


Note that
\begin{align*}
    \frac{\sum_{j=1}^d \sigma_j^{t} }{\sqrt{\sum_{j=1}^d \sigma_j^{2t}}} = \frac{1-\alpha^d}{1-\alpha} \sqrt{\frac{1-\alpha^2}{1-\alpha^{2d}}} = \sqrt{\frac{1+\alpha}{1-\alpha}}  \sqrt{\frac{1-\alpha^d}{1+\alpha^d}} 
    ~\in~ \left[1, \sqrt{\frac{1+\alpha}{1-\alpha}} \right].
\end{align*}
Therefore, by definition of $\lambda$ in~\eqref{eq:beta_t>2}, whenever $s/2 \geq \sqrt{\dfrac{1+\alpha}{1-\alpha}}  \sqrt{\dfrac{1-\alpha^d}{1+\alpha^d}} $, we have $\lambda = 0$ and
\begin{align*}
    \epsilon^*(s,t,\Sigma) \asymp \nu^t = 
    \left((\sigma\alpha)^{2t}\frac{1-\alpha^{2td}}{1-\alpha^{2t}}\right)^{1/2}
\end{align*}
Otherwise, we have
\begin{align*}
    s/2 = \frac{\sum_{j=1}^d \sigma_j^{t} \exp\left(-\beta/\sigma_j^2\right)}{\sqrt{\sum_{j=1}^d \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right)}} \asymp \frac{
        \displaystyle\sum_{j\leq j_*} \sigma_j^{t} 
        + \sum_{j> j_*} \sigma_j^{t} \exp\left(-\beta/\sigma_j^2\right)
        }{
        \sqrt{\displaystyle\sum_{j\leq j_*} \sigma_j^{2t} 
        + \sum_{j>j_*} \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right)}}.
\end{align*}
Moreover, for some $w \in \left[\exp\left(-\beta/\sigma_d^2\right), e^{-1}\right]$ we have
\begin{align*}
    \sum_{j> j_*} \sigma_j^{t} \exp\left(-\beta/\sigma_j^2\right) 
    = w \sum_{j> j_*} \sigma_j^{t} 
    = w \cdot  \frac{\alpha^{t(j_*+1)}-\alpha^{t(d+1)}}{1-\alpha^t} 
    \leq w \cdot  \frac{\alpha^{t}-\alpha^{t(j_*+1)}}{1-\alpha^t} 
\end{align*}


%let $j'$ be such that $s/2 = \sqrt{\dfrac{1+\alpha}{1-\alpha}}  \sqrt{\dfrac{1-\alpha^{j'}}{1+\alpha^{j'}}}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Moreover, we always have that 
$$ \nu^t = \sum\limits_{j=1}^d \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right) \asymp_t \sum\limits_{j\leq j_1} \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right) = \sqrt{\sum_{j=1}^d \alpha^{2t j}} = \sqrt{\frac{\alpha^{2t} - \alpha^{2t(d+1)}}{1-\alpha^{2t}}} \asymp \sqrt{\frac{\alpha^{2t}}{1-\alpha^{2t}}} \quad \text{ since } \alpha^{td} \leq \alpha^t/4.$$
If $s\geq C\sqrt{j_1}$, then $\lambda = 0$ and $\epsilon^*(s,t,\Sigma) \asymp \sqrt{\frac{\alpha^{2t}}{1-\alpha^{2t}}}.$ 
Otherwise, 
$$\epsilon^*(s,t,\Sigma) \asymp \sqrt{\frac{\alpha^{2t}}{1-\alpha^{2t}}} + \alpha^t s \log^{t/2}\left(C\sqrt{j_1}/s\right) \asymp \sqrt{\frac{\alpha^{2t}}{1-\alpha^{2t}}} + \alpha^t s \log^{t/2}\left(\frac{C}{s\log (1/\alpha)}\right).$$


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ù



\begin{tabular}{|c|c|c|c|c|c|cc|c|}
\cline{1-3} \cline{5-8}
If $t \in E$  
& $s\leq \sqrt{d}$ 
& $s > \sqrt{d}$ 
& 
& If $t \notin E$ 
& $s\leq \sqrt{d} $ (LB)
& $s\leq \sqrt{d}$ (UB) 
& $s > \sqrt{d}$ \rule[-2ex]{0pt}{6ex}  \\
\cline{1-3} \cline{5-8}
$\mathcal{R}_{s,d}^{1/2}(\sigma,t)$ 
& $\sigma s^{1/t} \sqrt{\log(1+d/s^2)}$  
& $\sigma d^{1/2t}$ 
&
&$\mathcal{R}_{s,d}^{1/2}(\sigma,t)$ 
&\multicolumn{1}{l|}{} 
&\rule[-2ex]{0pt}{6ex}  \\
\cline{1-3} \cline{5-8}
$\epsilon^*(s,t,\sigma^2I_d)$  
& $\sigma s^{1/t} \sqrt{\log\left(1+d/s^2\right)}$ 
& $\sigma d^{1/2t}$ 
&
& $\epsilon^*(s,t,\sigma^2I_d)$ 
&\multicolumn{1}{l|}{} 
&\rule[-2ex]{0pt}{6ex}  \\
\cline{1-3} \cline{5-8}
\end{tabular}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\begin{tabular}{|l|l|l|l|}
\hline
$t \notin E$ 
& $s > \sqrt{d}$ (Lower bound)   
& \multicolumn{1}{l|}{$s \leq \sqrt{d}$ (Upper Bound)}        
& $s \leq \sqrt{d}$    
\rule[-2ex]{0pt}{6ex}
\\ \hline
$\mathcal{R}_{s,d}^{1/2}(\sigma,t)$        
& R geq sqrt d 
& \multicolumn{1}{l|}{R leq sqrt d lb} 
& R geq sqrt d UB 
\rule[-2ex]{0pt}{6ex}
\\ \hline
$\epsilon^*(s,t,\sigma^2I_d)$, $t < 2$ 
& $\sigma^t d^{t/4} s^{1-t/2}$
& \multicolumn{2}{c|}{ \multirow{2}{*}{ $\sigma^t s \log^{t/2}\left(\dfrac{2\sqrt{d}}{s}\right)$}} 
\rule[-2ex]{0pt}{6ex}\\ 
\cline{1-1}\cline{4-4}
$\epsilon^*(s,t,\sigma^2I_d)$, $t > 2$ 
& $\sigma^t \sqrt{d}$
& \multicolumn{2}{c|}{} 
\rule[-2ex]{0pt}{6ex}\\ \hline
\end{tabular}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{center}
    \begin{tabular}{|c|c|c|}
    \hline
    $\epsilon^*(s,t,\sigma^2 I_d)^t$ & If $t \leq 2$ & If $t \geq 2$ \rule[-2ex]{0pt}{6ex} \\
    \hline
    If $s \geq C\sqrt{d}$ & $\sigma^t d^{t/4} s^{1-t/2}$ & $\sigma^t \sqrt{d}$ \rule[-2ex]{0pt}{6ex}\\
    \hline
    If $s < C\sqrt{d}$ & $\sigma^t s \log^{t/2}\left(\dfrac{2\sqrt{d}}{s}\right)$ & $\sigma^t s \log^{t/2}\left(\dfrac{2\sqrt{d}}{s}\right)$\rule[-2ex]{0pt}{6ex}\\
    \hline
\end{tabular}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{align*}
    \mathcal R_{s,d}(\sigma,t) \asymp \begin{cases}\sigma^2 s^{2/t} \log(1+d/s^2) & \text{ if  } s \leq \sqrt{d}\\
    \sigma^2 d^{1/t} & \text{ if } s > \sqrt{d} \text{ and $t$ is an even integer.}\end{cases}
\end{align*}


If $t$ is not an even integer, and $s>\sqrt{d}$, then the minimax estimation rate satisfies
\begin{align*}
    c \sigma^2 s^{2/t} \log^{1-2t}\!\Big(1+\frac{s^2}{d}\Big) \leq \mathcal R_{s,d}(\sigma,t) \leq \bar c\sigma^2 s^{2/t} \log^{-1}\!\Big(1+\frac{s^2}{d}\Big)
\end{align*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{enumerate}
    \item By Jensen's inequality, we have $\mathbb E |Y|^\alpha \leq \mathbb E^{\alpha/4} |Y|^4 \leq 3^{\alpha/4} \leq 3$.
    \item
By integration by parts, we have 
\begin{align*}
    \int_x^\infty y^\alpha e^{-y^2/2} dy &= x^{\alpha-1} e^{-x^2/2} + (\alpha\!-\!1)\! \int_x^{\infty} \! y^{\alpha-2} e^{-y^2/2} dy\\
    &\leq x^{\alpha-1} e^{-x^2/2} + \frac{1}{2} \int_x^\infty y^\alpha e^{-y^2/2} dy ~~ \text{using that $y^2 \geq \alpha-1$ over $[x,+\infty)$},\\
    \text{so that } \quad 
        \mathbb E \big[ |Y|^\alpha \mathbb 1_{|Y|\geq x}\big] &= 2 \int_x^\infty y^\alpha e^{-y^2/2} dy \leq 4x^{\alpha-1} e^{-x^2/2}.
\end{align*}
\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

, we have
We let $\lambda>0$ be the unique solution to the equation
\begin{equation}\label{eq:def_lambda_infty}
    \sum_{j=1}^d e^{-\lambda^2/2\sigma_j^2} = 1 \ju{check.}
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 define 
\vspace{-2mm}
\begin{align*}
    \pi_j = \frac{2\sigma_j^2e^{-\lambda^2/\sigma_j^2}}{\sqrt{\sum_{k=1}^d \sigma_j^4 e^{-\lambda^2/\sigma_j^2}}}, \quad \text{ so that } \sum_{j=1}^d \pi_j=1.
\end{align*}
We have 
\begin{align*}
    \nu = \sqrt{\sum_{k=1}^d \sigma_j^4 e^{-\lambda^2/\sigma_j^2}} = \sqrt{\sum_{k=1}^d \frac{\pi_j}{2}\sigma_j^2 \nu}, \text{ so that } \nu = \sum_{k=1}^d \frac{\pi_j}{2}\sigma_j^2 
\end{align*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We now impose that $2 c^2 \leq 1$ and we define $f(u) = u^{1-\delta}$ where $\delta = 2c^2 \in [0,1]$. 
By concavity of $f$, we have
\begin{align*}
    \sum_{j=1}^d \pi_j^{2-2c^2} - \pi_j^2 &= \mathbb E_{p} f(\pi_p) - \sum_{j=1}^d \pi_j^2 \leq f\left(\mathbb E_{p} \pi_p\right) - \sum_{j=1}^d \pi_j^2 = \alpha^{1-\delta} - \alpha
\end{align*}
where $\alpha = \sum_{j=1}^d \pi_j^2 \in (0,1)$. It is clear that the family of functions $\left(\alpha \mapsto \alpha^{1-\delta}\right)_{\delta>0}$ uniformly converges to the identity function over $[0,1]$ as $\delta \to 0$. 
Therefore, for any small constant $c'$ depending only on $\eta$, there exists a constant $\delta>0$ depending only on $\eta$ such that $\forall \alpha \in [0,1]: |\alpha^{1-\delta} - \alpha| \leq c'$. 
Fixing this constant $\delta>0$ provides a choice of $c>0$ ensuring that our prior is indistinguishable from $\mathbb P_0$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

, noting in the latter case that the term $1 \land \frac{\sigma_j^4}{x^{4-t} \nu^t(x)}$ from equation~\eqref{eq:def_f_ellt} always simplifies as $\frac{\sigma_j^4}{x^{4-t} \nu^t(x)}$ since we must have
$$\sum_{j\leq j_*(x)} 1 \land \frac{\sigma_j^4}{x^{4-t} \nu^t(x)} + \sum_{j>j_*(x)} \frac{\sigma_j^t}{\nu^t(x)} \exp\!\bigg(\!\!-\frac{x^2}{\sigma_j^2}+1\bigg) = \frac{1}{2}.$$

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Lower bounds for $t = \infty$}
To prove the lower bound, we once again use Le Cam's two points method with the following prior distribution over the parameter space $\Theta = \R^d$. 
We recall the definition of $\lambda$ in~\eqref{eq:def_lambda_infty} and set 
\begin{equation}\label{eq:def_pi_infty}
    \pi_j := e^{-\lambda^2/\sigma_j^2}, \quad \forall j \in [d].
\end{equation}
For a sufficiently small absolute constant 
$c>0$, we define a random vector $\theta \in \R^d$ whose coordinates $\theta_j$ satisfy $\forall j \in [d]: \theta_j = c\lambda \mathbb 1_{j=p}$, where $p$ is a random variable taking its values in $\{1,\dots,d\}$, and such that $\forall j \in [d]: \mathbb P(p=j) = \pi_j$. 
Equivalently, we will write $p \sim \operatorname{Mult}((\pi_1,\dots, \pi_d),1)$, where for any probability vector $\pi = (\pi_1,\dots, \pi_d) \in \R_+^{d}$ such that $\sum_{j=1}^d \pi_j = 1$, the notation $\operatorname{Mult}((\pi_1,\dots, \pi_d),1)$ denotes the multinomial distribution with parameters $\pi$ and $1$. 
Note that $\theta$ is $1$-sparse almost surely, and that its unique non-zero coordinate has magnitude~$c\lambda$. 
Note that in our prior, the perturbation $+c\lambda$ is always positive, which allows us to derive the following corollary:

%%%%%%%%%%%%%%%%%%%%%%%%
\begin{center}
    \begin{tabular}{|c|c|c|c|}
    \hline
    $\epsilon^*(s,t,\sigma^2 I_d)^t$ & If $t \leq 2$ & If $t \geq 2$ & If $t=\infty$ \rule[-2ex]{0pt}{6ex} \\
    \hline
    If $s \geq C\sqrt{d}$ & $\sigma^t d^{t/4} s^{1-t/2}$ & $\sigma^t \sqrt{d}$ & $\sigma\sqrt{\log(d)}$ \rule[-2ex]{0pt}{6ex}\\
    \hline
    If $s < C\sqrt{d}$ & $\sigma^t s \log^{t/2}\left(\dfrac{2\sqrt{d}}{s}\right)$ & $\sigma^t s \log^{t/2}\left(\dfrac{2\sqrt{d}}{s}\right)$ & $\sigma\sqrt{\log(d)}$ \rule[-2ex]{0pt}{6ex}\\
    \hline
\end{tabular}
\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Variances decreasing at least exponentially}
Assume that $t \geq 2$. 
If $\sigma_d \geq \frac{1}{4}$, then we are back to the isotropic case and $\epsilon^*(s,t,\Sigma) \asymp \epsilon^*(s,t, I_d)$. 
Otherwise, we have $\sigma_d < \frac{1}{4}$. 
Let $j_0 = \min \left\{j ~\big|~ \sigma_j < 1/2\right\}$ and 
$j_1 = \min \left\{j ~\big|~ \sigma_j < 1/4\right\}$. 
%By homogeneity, assume that $\sigma=1$.
Note that we have $1 \leq j_0 \leq j_1$ by monotonicity of the $(\sigma_j)_j$.
We will use the following relations, which are due to the convexity of $\phi$, and to the fact that $\phi$ is increasing and satisfies $\phi(0)=0$:
\begin{align}
    &\phi(j_1 +\ell)  \geq \phi(j_1) + \ell \phi'(j_1), \quad \forall \ell \geq 0,\label{eq:phi_cvx_1}\\
    &\phi(j) \leq \frac{\phi(j_0)}{j_0} \!\cdot \! j, \quad \forall j \leq j_0,\label{eq:phi_cvx_2}\\
    &\phi'(j_1) \geq \frac{\phi(j_1)}{j_1} \geq \frac{\phi(j_0)}{j_0}.\label{eq:phi_cvx_3}
\end{align}
The goal will be to prove that $\sum\limits_{j=1}^d \sigma_j^t \exp\left(-\beta/\sigma_j^2\right) \asymp_t \sum\limits_{j < j_1} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right)$, 
in other words, that we can only restrict our analysis to $\{0,\dots,j_1\!-\!1\}$, which is the largest set where the variances can be considered almost constant: $\forall j \in \{0,\dots,j_1\!-\!1\}: \sigma_j \in [1/4,1]$. 
To do so, our strategy is to justify the following relation, which clearly implies the latter one: 
\begin{align}
    \sum_{j\geq j_1} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right) \lesssim \sum_{j < j_0} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right). \label{eq:strategy}
\end{align}
To control the left hand side of~\eqref{eq:strategy}, we can write:
\begin{align*}
    \sum_{j \geq j_1} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right) &= \sum_{j \geq j_1} \exp\left(-t\phi(j) -\beta/\sigma_j^2\right)\\
    &\leq \exp\left(-t\phi(j_1) - \beta/\sigma_{j_1}^2 \right)\sum_{\ell \geq0} \exp(-t \ell \phi'(j_1) ) \\
    & \leq \frac{\exp\left(-t\phi(j_1) - \beta/\sigma_{j_1}^2\right)}{1 - \exp(-t \phi'(j_1))}. %\\
    %& \asymp \sigma_{j_1}^t \exp(-\beta/\sigma_{j_1}^2).
\end{align*}
To control the right-hand side of~\eqref{eq:strategy}, we can write
\begin{align*}
    \sum_{j < j_0} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right) 
    &\geq \exp\left(-\beta/\sigma_{j_1}^2\right) \sum_{j < j_0} \exp\left(- t\frac{\phi(j_0)}{j_0} \!\cdot \! j\right) \\
    & = \exp\left(-\beta/\sigma_{j_1}^2\right) \frac{1 - \exp\left(- t\frac{\phi(j_0)}{j_0} \!\cdot \! j_0\right)}{1-\exp\left(- t\frac{\phi(j_0)}{j_0}\right)} \\
    &\geq \exp\left(-\beta/\sigma_{j_1}^2\right) \frac{1-2^{-t}}{1-\exp\left(- t\frac{\phi(j_0)}{j_0}\right)} \text{ by definition of } j_0\\
    & \geq  \exp\left(-\beta/\sigma_{j_1}^2\right) \frac{1-2^{-t}}{1-\exp\left(- t \phi'(j_1)\right)} \text{ by \eqref{eq:phi_cvx_3}}. 
\end{align*}
Therefore, we always have $\sum\limits_{j=1}^d \sigma_j^t \exp\left(-\beta/\sigma_j^2\right) \asymp_t \sum\limits_{j\leq j_1} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right)$. 
Proceeding similarly, we can also get $\sum\limits_{j=1}^d \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right) \asymp_t \sum\limits_{j\leq j_1} \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right)$. 
Now, it follows that
\begin{align*}
    s/2 \asymp \frac{\sum\limits_{j\leq j_1} \sigma_j^t \exp\left(-\beta/\sigma_j^2\right)}{\sqrt{\sum\limits_{j \leq j_1} \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right)}} \asymp \sqrt{j_1} \exp\left(-\beta/C'\alpha^2\right), \quad \text{ hence } \beta = C'\alpha^2 \log\left(C\sqrt{j_1}/s\right),
\end{align*}
for some constants $C,C'$ depending only on $t$. 
Moreover, $\nu^{2t} \asymp \sum\limits_{j \leq j_1} \sigma_j^{2t} \exp\left(-\beta/\sigma_j^2\right)$. 
We exactly recover the analysis of the isotropic case from Subsection~\ref{subsec:proof_isotropic}.
In other words, it holds that $\epsilon^*(s,t,\Sigma) \asymp \epsilon^*(s,t,\alpha^2 I_{j_1})$, where by definition of $j_1$, we have $j_1 \asymp \log^{-1}(1/\alpha)$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Note that this result encompasses the case of exponentially decreasing variances. 
More precisely, let $\alpha \in (0,1]$ and assume that $\forall j \in \{0,\dots d\}: \sigma_j = \alpha^j$. 
Let $j_0 = \min\big\{j \in [d] ~\big|~ \alpha^{j} < \alpha/2\big\}$ if this minimum is taken over a non-empty set, and set $j_0 = d+1$ otherwise.
The case where $t=2$ has been examined in~\cite{laurent2012non}. 
Here, we assume that $t \geq 2$. 
Then the minimax separation radius satisfies
\begin{align}
    \forall t \geq 2: ~~ \epsilon^*(s,t,\Sigma) \asymp \epsilon^*(s,t,\alpha^2 I_{j_0}) \asymp \begin{cases}\alpha j_0^{1/2t} & \text{ if } s \geq C \sqrt{j_0},\\
    \alpha^t s \log^{t/2}\left(\dfrac{2\sqrt{j_0}}{s}\right) & \text{ otherwise.}
    \end{cases}
    \label{eq:rate_exponential}
\end{align}
Note that this result encompasses the isotropic case from Subsection~\ref{subsec:isotropic}.
For non-pathological decays of the values $\sigma_j$'s, that is, for $\alpha \leq 1-\delta$ where $\delta>0$ is some fixed constant, the index $j_0$ will typically be a constant depending on $\delta$.
Namely: $j_0 \leq \log_{\alpha^{-1}} (2) \leq \log_{(1-\delta)^{-1}} (2)$. 
Therefore, as soon as $s$ is greater than a constant (depending on $\delta$), the minimax separation radius will further simplify as $\epsilon^*(s,t,\Sigma) \asymp_\delta \alpha = \sigma_1$, regardless of the sparsity.
This makes intuitive sense: 
When the $\sigma_j$'s decay exponentially fast, the intrinsic dimension of the data, given by $d_{intrinsic} = \operatorname{Tr}(\Sigma^{t/2}) / \sqrt{\operatorname{Tr}(\Sigma^t)}$, is of the order of a constant. 
Therefore, sparsity should not be relevant if $s \geq \sqrt{d}_{intrinsic} = Cste$ (see the discussion in Subsection~\ref{subsec:L2_separation}).
\vspace{2mm}

However, the rate can be more subtle if $\alpha$ approaches $1$, and equation~\eqref{eq:rate_exponential} reveals that whenever $\sigma_j = \alpha^j$ for $j=0\dots,d$, the testing problem is essentially as difficult in the isotropic case with covariance matrix $\alpha^2 I_{j_0}$. 
Here, the dimension $j_0$ can understood as the size of the set $\{0,\dots j_0\}$ on which the values $\sigma_j$ can be considered as constant: $\sigma_j \in \left[\frac{1}{2}\sigma_1, \sigma_1\right], \forall j \in \{0,\dots, j_0\}$.





